Automatic Image Filtering on Social Networks Using Deep Learning and Perceptual Hashing During Crises

The extensive use of social media platforms, especially during disasters, creates unique opportunities for humanitarian organizations to gain situational awareness and launch relief operations accordingly. In addition to the textual content, people post overwhelming amounts of imagery data on social networks within minutes of a disaster hit. Studies point to the importance of this online imagery content for emergency response. Despite recent advances in the computer vision field, automatic processing of the crisis-related social media imagery data remains a challenging task. It is because a majority of which consists of redundant and irrelevant content. In this paper, we present an image processing pipeline that comprises de-duplication and relevancy filtering mechanisms to collect and filter social media image content in real-time during a crisis event. Results obtained from extensive experiments on real-world crisis datasets demonstrate the significance of the proposed pipeline for optimal utilization of both human and machine computing resources.

==> discussion_old.tex <==
\section{Discussion}

%\textcolor{red}{\bf TODO: Firoj, please put significance testing results here...}

\textcolor{red}{\bf TODO: These paragraphs are copied from different parts of the experiments section. So, the redundancy between the two sections needs to be consolidated. The disconnected paragraphs need to be connected. AUC plots need to be explained a little bit in more detail.}

Although we observe an overall decrease in all performance scores as compared to the S.1 setting, we believe the performance results for the S.2 setting are more trustworthy due to the following observation. In the S.1 setting, due to the appearance of duplicate or near-duplicate images both in training and test sets, the classifier gets biased and thus shows high but unreliable performance.


Even though the training data for S.1 and S.3 are not exactly the same, we can still try to compare the performance of the damage assessment model with (i.e., S.1) and without (i.e., S.3) irrelevant images. As we see from S.1 and S.3 columns of Table~\ref{tbl:classification_report}, the scores for none category in S.3 are lower than those in S.1 whereas the scores for severe and mild categories in S.3 are higher than those in S.1. After macro averaging the scores for all categories, we see that overall F1-score for S.3 is 0.01 higher the overall F1-score for S.2. Though macro-averaged AUC scores seem to be the same. However, we already know from previous section that having duplicate or near-duplicate images in the training set yield untrustworthy model results. Hence, we do not intend to elaborate any further on this comparison.


If we compare the performance results for S.3 (free of irrelevant but has duplicates) and S.4, we see that removing duplicate images from the training data eliminates the artificial increase in the performance scores, which is in agreement with the trend observed between S.1 and S.2 settings.

More interestingly, we can try to see the benefit of removing irrelevant images when the data is already free of duplicates. That is, we can try to compare the results of the settings S.2 (without duplicates, with irrelevant) and S.4 (without duplicates, without irrelevant), even though the training data for both settings are not exactly the same. At the category level, we observe a similar behavior as before, where the scores for none category in S.4 are slightly lower than those in S.2 while the scores for severe and mild categories in S.4 are slightly higher than those in S.2. If we compare the macro-averaged F1-scores, we see that S.4 outperforms S.2 by a small margin of 0.02. In order to assess whether this difference in F1-score between S.2 and S.4 is significant or not, we perform a permutation test (or sometimes called a randomization test) in the following manner. We randomly shuffle 1,000 times the input test image labels and the output model predictions within a common pool of S.2 and S.4 datasets. Then for each shuffle, we compute the difference in F1-scores for S.2 and S.4 settings. Eventually, we compare the actual observed F1-score distance against the distribution of such sampled 1,000 F1-score differences to see if the observed value is statistically significantly away from the mean of the sample distribution. In our case, we get $p=0.077$, which is not statistically significant but shows a certain trend toward significance.

Finally, Figure~\ref{fig:auc} shows the precision-recall curves for all four settings.


